Design Challenges in Low-resource Cross-lingual Entity Linking

Cross-lingual Entity Linking (XEL), the problem of grounding mentions of entities in a foreign language text into an English knowledge base such as Wikipedia, has seen a lot of research in recent years, with a range of promising techniques. However, current techniques do not rise to the challenges introduced by text in low-resource languages (LRL) and, surprisingly, fail to generalize to text not taken from Wikipedia, on which they are usually trained. This paper provides a thorough analysis of low-resource XEL techniques, focusing on the key step of identifying candidate English Wikipedia titles that correspond to a given foreign language mention. Our analysis indicates that current methods are limited by their reliance on Wikipedia's interlanguage links and thus suffer when the foreign language's Wikipedia is small. We conclude that the LRL setting requires the use of outside-Wikipedia cross-lingual resources and present a simple yet effective zero-shot XEL system, QuEL, that utilizes search engines query logs. With experiments on 25 languages, QuEL~shows an average increase of 25\% in gold candidate recall and of 13\% in end-to-end linking accuracy over state-of-the-art baselines.

==> sections/1.5-background.tex <==

\section{Problem Formulation}
We formalize the XEL problem as follows. 
Given a mention $m$ in a document written in the source language $SL$, a XEL system aims to link it to the corresponding English Wikipedia entity $e$. 
The task breaks down into two processes: candidate generation and candidate ranking.
Given $m$, we first generate a list of all possible  English Wikipedia candidates $C(m)$ = $\{e_1, e_2, e_3, ...\}$, with the goal to include the gold entity $e$ in $C(m)$.
Further, we compute weighting scores $W(e_i, m), \forall e_i \in C(m)$ to rank candidates $C(m)$ and select the most likely one.



==> tables/22langs.tex <==
{
\begin{table}[t]
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\multirow{2}{*}{ Model } & \multicolumn{2}{c}{ ta } & \multicolumn{2}{c}{ zu } & \multicolumn{2}{c}{ ak } & \multicolumn{2}{c}{ am } & \multicolumn{2}{c}{ hi } & \multicolumn{2}{c}{ id } & \multicolumn{3}{c}{ es } & \multicolumn{3}{c}{ ar } & \multicolumn{3}{c}{ sw } & \multicolumn{3}{c}{ wo } & \multicolumn{3}{c}{ vi } & \multicolumn{3}{c}{ th } & \multicolumn{3}{c}{ bn } & \multicolumn{3}{c}{ tl } & \multicolumn{3}{c}{ hu } & \multicolumn{2}{c}{ zh } & \multicolumn{2}{c}{ fa } & \multicolumn{2}{c}{ ru } & \multicolumn{2}{c}{ om } & \multicolumn{2}{c}{ ti } & \multicolumn{2}{c}{ si } & \multicolumn{2}{c}{ rw } & \multicolumn{2}{c}{ ilo } & \multicolumn{2}{c}{ or } & \multicolumn{2}{c}{ som } \\
& H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@5 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all & H@1 & H@all \\
P(t|m) & 0.518 & 0.594 & 0.196 & 0.198 & 0.239 & 0.239 & 0.233 & 0.282 & 0.535 & 0.639 & 0.625 & 0.674 & 0.639 & 0.781 & 0.781 & 0.742 & 0.815 & 0.815 & 0.613 & 0.696 & 0.696 & 0.166 & 0.169 & 0.169 & 0.824 & 0.869 & 0.869 & 0.4 & 0.501 & 0.501 & 0.365 & 0.464 & 0.464 & 0.614 & 0.653 & 0.653 & 0.525 & 0.664 & 0.664 & 0.614 & 0.832 & 0.661 & 0.761 & 0.539 & 0.574 & & & & & & & & & & & & & & \\
Chentse & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\
Hengji & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\
Neubig & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & 0.343 & 0.37 & 0.153 & 0.191 & & & & & & & & \\
Google top1 & 0.581 & 0.661 & 0.261 & 0.38 & 0.551 & 0.61 & 0.345 & 0.36 & 0.622 & 0.718 & 0.594 & 0.683 & 0.553 & 0.678 & 0.678 & 0.737 & 0.838 & 0.838 & 0.663 & 0.762 & 0.762 & 0.498 & 0.635 & 0.635 & 0.804 & 0.869 & 0.879 & 0.74 & 0.771 & 0.771 & 0.474 & 0.54 & 0.54 & 0.735 & 0.816 & 0.82 & 0.482 & 0.682 & 0.69 & 0.599 & 0.861 & & & & & & & 0.436 & 0.463 & 0.602 & 0.697 & & & & & & & & \\
Google top5 & 0.582 & 0.766 & 0.224 & 0.411 & 0.54 & 0.79 & 0.338 & 0.382 & 0.629 & 0.774 & 0.6 & 0.746 & 0.566 & 0.714 & 0.726 & 0.751 & 0.851 & 0.875 & 0.654 & 0.843 & 0.858 & 0.455 & 0.728 & 0.744 & 0.814 & 0.902 & 0.918 & 0.738 & 0.794 & 0.795 & 0.469 & 0.608 & 0.631 & 0.735 & 0.874 & 0.883 & 0.48 & 0.739 & 0.778 & 0.738 & 0.88 & & & & & & & 0.456 & 0.495 & 0.627 & 0.739 & & & & & & & & \\
Google t5 + P(t|m) & 0.564 & 0.766 & 0.218 & 0.411 & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & 0.63 & 0.739 & & & & & & & & \\
Google + trans & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\
Google + bert & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\
\end{tabular}
\end{table}
}

==> tables/framework.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{tables/flow.pdf}
\vspace{-0.4cm}
\caption{An overview of our proposed \modelname~XEL method. Given a source language mention, the system runs it through language-specific morphological normalization, pivoting techniques, and name transliteration models for query inputs in query log and Google Map. The candidates generated from each component is ranked using cross-checking to re-weight, along with M-BERT for contextual disambiguation.
Note that the example sentence is not supported by Google Translation, and the meaning remains unknown to us.}
\vspace{-0.2cm}
\label{fig:framework}
\end{figure*}

==> tables/native-speaker.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{tables/native_speaker.pdf}
\vspace{-0.4cm}
\vspace{-0.2cm}
\caption{Native speaker number (in million) for each language, data retrieved from Wikipedia.}
\label{fig:native_speaker}
\end{figure*}
